GADMM: Fast and Communication Efficient Framework for Distributed Machine Learning

When the data is distributed across multiple servers, lowering the communication cost between the servers (or workers) while solving the distributed learning problem is an important problem and is the focus of this paper. In particular, we propose a fast, and communication-efficient decentralized framework to solve the distributed machine learning (DML) problem. The proposed algorithm, Group Alternating Direction Method of Multipliers (GADMM) is based on the Alternating Direction Method of Multipliers (ADMM) framework. The key novelty in GADMM is that it solves the problem in a decentralized topology where at most half of the workers are competing for the limited communication resources at any given time. Moreover, each worker exchanges the locally trained model only with two neighboring workers, thereby training a global model with a lower amount of communication overhead in each exchange. We prove that GADMM converges to the optimal solution for convex loss functions, and numerically show that it converges faster and more communication-efficient than the state-of-the-art communication-efficient algorithms such as the Lazily Aggregated Gradient (LAG) and dual averaging, in linear and logistic regression tasks on synthetic and real datasets. Furthermore, we propose Dynamic GADMM (D-GADMM), a variant of GADMM, and prove its convergence under the time-varying network topology of the workers.

==> convRate.tex <==


Now, we provide the convergence rate of GADMM. First, it is worth mentioning that the convergence rate of Gauss-Seidel ADMM for sum of two separable convex functions has been studied in~\citep{lions1979splitting,he20121,he2015non}. In particular, \citep{he20121} shows a convergence rate of $O(1/k)$. Moreover, \citep{deng2017parallel} improves that results and shows a convergence rate of $o(1/k)$. In the following result, we leverage and extend the proof of $o(1/k)$ convergence rate in \cite[Sec. 5]{deng2017parallel} to show that GADMM achieves the same convergence~rate. We start by introducing the following Lemma due to \citep{deng2017parallel}. 

\begin{lemma}\label{lemma:convRate}
If a sequence $\{a_k\} \subseteq R$ is such that   
%\begin{enumerate}
$a_k \geq 0$,
$\sum_{k=1}^\infty a_k < +\infty$,
 and $a_k$ is monotonically non-increasing, 
%\end{enumerate}
then it holds that $a_k=o(1/k)$.
\end{lemma}
\begin{proof}
The proof of Lemma~\ref{lemma:convRate} follows the same lines of the proof in \cite[Lemma 1.2]{deng2017parallel}. 
\end{proof}
The result in Lemma \ref{lemma:convRate} says that for a summable, non-negative, and monotonic $a_k$, $a_k$ will converge faster than $1/k$. This will be used in the following result to prove the improved convergence rate of $o(1/k)$.
\if0
\colr{Next, we establish the convergenc rate for the proposed GADMM algorithm. }}
\colr{In order to prove the convergence rate, we define a compact notation with $\bbw\in\mathbb{R}^{2Nd\times 1}$ as  $\mathbf{w}=[\boldsymbol{\theta}_1^T \boldsymbol{\theta}_2^T \ \cdots\  \boldsymbol{\theta}_N^T \ \boldsymbol{\lambda}_1^T \ \boldsymbol{\lambda}_2^T\ \cdots \ \boldsymbol{\lambda}_N^T]^T$ for all $n$. Utilizing this notation, we can write the Lyapunov function in \eqref{lyapEq} as follows.
%
\begin{align}\label{notation}
V_k=\norm{\mathbf{w}_k-\mathbf{w}^\star}_H^2
\end{align}
where
\begin{align}
\bbH=\begin{bmatrix} 
\bbA & \textbf{0}\\
\textbf{0}& \bbB\\
\end{bmatrix}; 
\bbA=\begin{bmatrix} 
\textbf{0} & \\
& 2\rho\bbI\\
&& \textbf{0}\\
&&& 2\rho\bbI\\
&&&& \ddots\\
&&&&& \textbf{0}\\
&&&&&& \bbI\\
\end{bmatrix};\bbB=\begin{bmatrix} 
(1/\rho)\bbI & \\
& (1/\rho)\bbI\\
&& \ddots\\
&&& (1/\rho)\bbI\\
&&&& \textbf{0}\\
\end{bmatrix}.
\end{align}
Note that here $\bbH\in \mathbb{R}^{2Nd\times 2Nd}$, $\bbA\in \mathbb{R}^{Nd\times Nd}$, and $\bbB\in \mathbb{R}^{Nd\times Nd}$. (Anis, please double check this. We will use the notation $\bbw_n$) to derives the convergence rate for the proposed algorithm. We use the the term $\|\bbw_k-\bbw_{k+1}\|^2_{\bbH}$ as the measure to calculate the rate of convergence as motivated in \citep{deng2017parallel,he2015non,he2015full} . }


\fi


\begin{theorem}
	GADMM achieves an $o(1/k)$ convergence rate which is the fastest rate among existing ADMM methods. In other words, $\boldsymbol{\theta}_{n}$ and $\boldsymbol{\lambda}_{n}$ converge at a rate of $o(1/k)$.
	\label{convRateProof}
\end{theorem}
\begin{proof}
The proof is provided in Appendix~\ref{ConvRate11}. The key idea is to show that the sequence of primal and dual optimality gaps generated by the propose algorithm satisfies the conditions of Lemma \ref{lemma:convRate}, hence GADMM iterates converges faster than $1/k$.

\end{proof}





\if0
Now, we provide the convergence rate of GADMM. First, it is worth mentioning that the convergence rate of Gauss-Seidel ADMM for sum of two separable convex functions has been studied in~\citep{lions1979splitting,he20121,he2015non}. In particular, \citep{he20121} shows a convergence rate of $O(1/k)$. Moreover, \citep{deng2017parallel} improves that results and shows a convergence rate of $o(1/k)$. In the following result, we leverage and extend the proof of $o(1/k)$ convergence rate in \cite[Sec. 5]{deng2017parallel} to show that GADMM achieves the same convergence~rate. We start by introducing the following Lemma due to \citep{deng2017parallel}. 

\begin{lemma}\label{lemma:convRate}
If a sequence $\{a_k\} \subseteq R$ is such that   
%\begin{enumerate}
$a_k \geq 0$,
$\sum_{k=1}^\infty a_k < +\infty$,
 and $a_k$ is monotonically non-increasing, 
%\end{enumerate}
then it holds that $a_k=o(1/k)$.
\end{lemma}
\begin{proof}
The proof of Lemma~\ref{lemma:convRate} follows the same lines of the proof in \cite[Lemma 1.2]{deng2017parallel}. 
\end{proof}
\colb{The result in Lemma \ref{lemma:convRate} says that for a summable, non-negative, and monotonic $a_k$, $a_k$ will converge faster than $1/k$. This will be used in the following result to prove the improved convergence rate of $o(1/k)$. \colr{Next, we establish the convergenc rate for the proposed GADMM algorithm. }}
\colr{In order to prove the convergence rate, we define a compact notation with $\bbw\in\mathbb{R}^{2Nd\times 1}$ as  $\mathbf{w}=[\boldsymbol{\theta}_1^T \boldsymbol{\theta}_2^T \ \cdots\  \boldsymbol{\theta}_N^T \ \boldsymbol{\lambda}_1^T \ \boldsymbol{\lambda}_2^T\ \cdots \ \boldsymbol{\lambda}_N^T]^T$ for all $n$. Utilizing this notation, we can write the Lyapunov function in \eqref{lyapEq} as follows.
%
\begin{align}\label{notation}
V_k=\norm{\mathbf{w}_k-\mathbf{w}^\star}_H^2
\end{align}
where
\begin{align}
\bbH=\begin{bmatrix} 
\bbA & \textbf{0}\\
\textbf{0}& \bbB\\
\end{bmatrix}; 
\bbA=\begin{bmatrix} 
\textbf{0} & \\
& 2\rho\bbI\\
&& \textbf{0}\\
&&& 2\rho\bbI\\
&&&& \ddots\\
&&&&& \textbf{0}\\
&&&&&& \bbI\\
\end{bmatrix};\bbB=\begin{bmatrix} 
(1/\rho)\bbI & \\
& (1/\rho)\bbI\\
&& \ddots\\
&&& (1/\rho)\bbI\\
&&&& \textbf{0}\\
\end{bmatrix}.
\end{align}
Note that here $\bbH\in \mathbb{R}^{2Nd\times 2Nd}$, $\bbA\in \mathbb{R}^{Nd\times Nd}$, and $\bbB\in \mathbb{R}^{Nd\times Nd}$. (Anis, please double check this. We will use the notation $\bbw_n$) to derives the convergence rate for the proposed algorithm. We use the the term $\|\bbw_k-\bbw_{k+1}\|^2_{\bbH}$ as the measure to calculate the rate of convergence as motivated in \citep{deng2017parallel,he2015non,he2015full} . }
\begin{theorem}
	GADMM achieves an $o(1/k)$ convergence rate which is the fastest rate among existing ADMM methods. {\color{blue}In other words, $\boldsymbol{\theta}_{n}$ and $\boldsymbol{\lambda}_{n}$ converge at a rate of $o(1/k)$. }
	\label{convRateProof}
\end{theorem}
\begin{proof}
The proof is provided in Appendix~\ref{ConvRate}. The key idea is to show that the sequence of primal and dual optimality gaps generated by the propose algorithm satisfies the conditions of Lemma \ref{lemma:convRate}, hence GADMM {\color{blue} iterates} converges faster than $1/k$.

\end{proof}
\fi

